Measurement of the branching fraction of the $B^{0}\rightarrow D_{s}^{+}\pi^{-}$ decay

A branching fraction measurement of the $B^{0}\rightarrow D_{s}^{+}\pi^{-}$ decay is presented using proton-proton collision data collected with the LHCb experiment, corresponding to an integrated luminosity of $5.0\,$fb$^{-1}$. The branching fraction is found to be ${\mathcal{B}(B^{0}\rightarrow D_{s}^{+}\pi^{-}) = (19.4 \pm 1.8\pm 1.3 \pm 1.2)\times 10^{-6}}$, where the first uncertainty is statistical, the second systematic and the third is due to the uncertainty on the $B^0 \to D^{-}\pi^{+}$, $D_{s}^{+}\rightarrow K^{+}K^{-}\pi^{+}$ and $D^{-}\rightarrow K^{+}\pi^{-}\pi^{-}$ branching fractions. This is the most precise single measurement of this quantity to date. As this decay proceeds through a single amplitude involving a $b \to u$ charged-current transition, the result provides information on non-factorisable strong interaction effects and the magnitude of the Cabibbo-Kobayashi-Maskawa matrix element $V_{ub}$. Additionally, the collision energy dependence of the hadronisation-fraction ratio $f_s/f_d$ is measured through $\bar{B}{}_{s}^{0}\rightarrow D_{s}^{+}\pi^{-}$ and $B^0 \to D^{-}\pi^{+}$ decays.

==> LHCb_Authorship_15-Jul-2020.tex <==
% LHCb collaboration author list
% Data extracted on July 15th, 2020 at 7:18pm for reference date 15-Jul-2020
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{31}$,
C.~Abell{\'a}n~Beteta$^{49}$,
T.~Ackernley$^{59}$,
B.~Adeva$^{45}$,
M.~Adinolfi$^{53}$,
H.~Afsharnia$^{9}$,
C.A.~Aidala$^{84}$,
S.~Aiola$^{25}$,
Z.~Ajaltouni$^{9}$,
S.~Akar$^{64}$,
J.~Albrecht$^{14}$,
F.~Alessio$^{47}$,
M.~Alexander$^{58}$,
A.~Alfonso~Albero$^{44}$,
Z.~Aliouche$^{61}$,
G.~Alkhazov$^{37}$,
P.~Alvarez~Cartelle$^{47}$,
S.~Amato$^{2}$,
Y.~Amhis$^{11}$,
L.~An$^{21}$,
L.~Anderlini$^{21}$,
A.~Andreianov$^{37}$,
M.~Andreotti$^{20}$,
G.~Anzivino$^{76}$,
F.~Archilli$^{16}$,
A.~Artamonov$^{43}$,
M.~Artuso$^{67}$,
K.~Arzymatov$^{41}$,
E.~Aslanides$^{10}$,
M.~Atzeni$^{49}$,
B.~Audurier$^{11}$,
S.~Bachmann$^{16}$,
M.~Bachmayer$^{48}$,
J.J.~Back$^{55}$,
S.~Baker$^{60}$,
P.~Baladron~Rodriguez$^{45}$,
V.~Balagura$^{11}$,
W.~Baldini$^{20}$,
J.~Baptista~Leite$^{1}$,
R.J.~Barlow$^{61}$,
S.~Barsuk$^{11}$,
W.~Barter$^{60}$,
M.~Bartolini$^{23,h}$,
F.~Baryshnikov$^{80}$,
J.M.~Basels$^{13}$,
G.~Bassi$^{28}$,
B.~Batsukh$^{67}$,
A.~Battig$^{14}$,
A.~Bay$^{48}$,
M.~Becker$^{14}$,
F.~Bedeschi$^{28}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{67}$,
V.~Belavin$^{41}$,
S.~Belin$^{26}$,
V.~Bellee$^{48}$,
K.~Belous$^{43}$,
I.~Belyaev$^{38}$,
G.~Bencivenni$^{22}$,
E.~Ben-Haim$^{12}$,
A.~Berezhnoy$^{39}$,
R.~Bernet$^{49}$,
D.~Berninghoff$^{16}$,
H.C.~Bernstein$^{67}$,
C.~Bertella$^{47}$,
E.~Bertholet$^{12}$,
A.~Bertolin$^{27}$,
C.~Betancourt$^{49}$,
F.~Betti$^{19,e}$,
M.O.~Bettler$^{54}$,
Ia.~Bezshyiko$^{49}$,
S.~Bhasin$^{53}$,
J.~Bhom$^{33}$,
L.~Bian$^{72}$,
M.S.~Bieker$^{14}$,
S.~Bifani$^{52}$,
P.~Billoir$^{12}$,
M.~Birch$^{60}$,
F.C.R.~Bishop$^{54}$,
A.~Bizzeti$^{21,r}$,
M.~Bj{\o}rn$^{62}$,
M.P.~Blago$^{47}$,
T.~Blake$^{55}$,
F.~Blanc$^{48}$,
S.~Blusk$^{67}$,
D.~Bobulska$^{58}$,
V.~Bocci$^{30}$,
J.A.~Boelhauve$^{14}$,
O.~Boente~Garcia$^{45}$,
T.~Boettcher$^{63}$,
A.~Boldyrev$^{81}$,
A.~Bondar$^{42}$,
N.~Bondar$^{37}$,
S.~Borghi$^{61}$,
M.~Borisyak$^{41}$,
M.~Borsato$^{16}$,
J.T.~Borsuk$^{33}$,
S.A.~Bouchiba$^{48}$,
T.J.V.~Bowcock$^{59}$,
A.~Boyer$^{47}$,
C.~Bozzi$^{20}$,
M.J.~Bradley$^{60}$,
S.~Braun$^{65}$,
A.~Brea~Rodriguez$^{45}$,
M.~Brodski$^{47}$,
J.~Brodzicka$^{33}$,
A.~Brossa~Gonzalo$^{55}$,
D.~Brundu$^{26}$,
A.~Buonaura$^{49}$,
C.~Burr$^{47}$,
A.~Bursche$^{26}$,
A.~Butkevich$^{40}$,
J.S.~Butter$^{31}$,
J.~Buytaert$^{47}$,
W.~Byczynski$^{47}$,
S.~Cadeddu$^{26}$,
H.~Cai$^{72}$,
R.~Calabrese$^{20,g}$,
L.~Calero~Diaz$^{22}$,
S.~Cali$^{22}$,
R.~Calladine$^{52}$,
M.~Calvi$^{24,i}$,
M.~Calvo~Gomez$^{83}$,
P.~Camargo~Magalhaes$^{53}$,
A.~Camboni$^{44}$,
P.~Campana$^{22}$,
D.H.~Campora~Perez$^{47}$,
A.F.~Campoverde~Quezada$^{5}$,
S.~Capelli$^{24,i}$,
L.~Capriotti$^{19,e}$,
A.~Carbone$^{19,e}$,
G.~Carboni$^{29}$,
R.~Cardinale$^{23,h}$,
A.~Cardini$^{26}$,
I.~Carli$^{6}$,
P.~Carniti$^{24,i}$,
K.~Carvalho~Akiba$^{31}$,
A.~Casais~Vidal$^{45}$,
G.~Casse$^{59}$,
M.~Cattaneo$^{47}$,
G.~Cavallero$^{47}$,
S.~Celani$^{48}$,
P.~Cenci$^{76}$,
J.~Cerasoli$^{10}$,
A.J.~Chadwick$^{59}$,
M.G.~Chapman$^{53}$,
M.~Charles$^{12}$,
Ph.~Charpentier$^{47}$,
G.~Chatzikonstantinidis$^{52}$,
M.~Chefdeville$^{8}$,
C.~Chen$^{3}$,
S.~Chen$^{26}$,
A.~Chernov$^{33}$,
S.-G.~Chitic$^{47}$,
V.~Chobanova$^{45}$,
S.~Cholak$^{48}$,
M.~Chrzaszcz$^{33}$,
A.~Chubykin$^{37}$,
V.~Chulikov$^{37}$,
P.~Ciambrone$^{22}$,
M.F.~Cicala$^{55}$,
X.~Cid~Vidal$^{45}$,
G.~Ciezarek$^{47}$,
F.~Cindolo$^{19}$,
P.E.L.~Clarke$^{57}$,
M.~Clemencic$^{47}$,
H.V.~Cliff$^{54}$,
J.~Closier$^{47}$,
J.L.~Cobbledick$^{61}$,
V.~Coco$^{47}$,
J.A.B.~Coelho$^{11}$,
J.~Cogan$^{10}$,
E.~Cogneras$^{9}$,
L.~Cojocariu$^{36}$,
P.~Collins$^{47}$,
T.~Colombo$^{47}$,
A.~Contu$^{26}$,
N.~Cooke$^{52}$,
G.~Coombs$^{58}$,
G.~Corti$^{47}$,
C.M.~Costa~Sobral$^{55}$,
B.~Couturier$^{47}$,
D.C.~Craik$^{63}$,
J.~Crkovsk\'{a}$^{66}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{57}$,
C.L.~Da~Silva$^{66}$,
E.~Dall'Occo$^{14}$,
J.~Dalseno$^{45}$,
C.~D'Ambrosio$^{47}$,
A.~Danilina$^{38}$,
P.~d'Argent$^{47}$,
A.~Davis$^{61}$,
O.~De~Aguiar~Francisco$^{61}$,
K.~De~Bruyn$^{77}$,
S.~De~Capua$^{61}$,
M.~De~Cian$^{48}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{18,d}$,
D.~De~Simone$^{49}$,
P.~De~Simone$^{22}$,
J.A.~de~Vries$^{78}$,
C.T.~Dean$^{66}$,
W.~Dean$^{84}$,
D.~Decamp$^{8}$,
L.~Del~Buono$^{12}$,
B.~Delaney$^{54}$,
H.-P.~Dembinski$^{14}$,
A.~Dendek$^{34}$,
X.~Denis$^{72}$,
V.~Denysenko$^{49}$,
D.~Derkach$^{81}$,
O.~Deschamps$^{9}$,
F.~Desse$^{11}$,
F.~Dettori$^{26,f}$,
B.~Dey$^{72}$,
P.~Di~Nezza$^{22}$,
S.~Didenko$^{80}$,
H.~Dijkstra$^{47}$,
V.~Dobishuk$^{51}$,
A.M.~Donohoe$^{17}$,
F.~Dordei$^{26}$,
M.~Dorigo$^{28,v}$,
A.C.~dos~Reis$^{1}$,
L.~Douglas$^{58}$,
A.~Dovbnya$^{50}$,
A.G.~Downes$^{8}$,
K.~Dreimanis$^{59}$,
M.W.~Dudek$^{33}$,
L.~Dufour$^{47}$,
V.~Duk$^{76}$,
P.~Durante$^{47}$,
J.M.~Durham$^{66}$,
D.~Dutta$^{61}$,
M.~Dziewiecki$^{16}$,
A.~Dziurda$^{33}$,
A.~Dzyuba$^{37}$,
S.~Easo$^{56}$,
U.~Egede$^{68}$,
V.~Egorychev$^{38}$,
S.~Eidelman$^{42,u}$,
S.~Eisenhardt$^{57}$,
S.~Ek-In$^{48}$,
L.~Eklund$^{58}$,
S.~Ely$^{67}$,
A.~Ene$^{36}$,
E.~Epple$^{66}$,
S.~Escher$^{13}$,
J.~Eschle$^{49}$,
S.~Esen$^{31}$,
T.~Evans$^{47}$,
A.~Falabella$^{19}$,
J.~Fan$^{3}$,
Y.~Fan$^{5}$,
B.~Fang$^{72}$,
N.~Farley$^{52}$,
S.~Farry$^{59}$,
D.~Fazzini$^{24,i}$,
P.~Fedin$^{38}$,
M.~F{\'e}o$^{47}$,
P.~Fernandez~Declara$^{47}$,
A.~Fernandez~Prieto$^{45}$,
F.~Ferrari$^{19,e}$,
L.~Ferreira~Lopes$^{48}$,
F.~Ferreira~Rodrigues$^{2}$,
S.~Ferreres~Sole$^{31}$,
M.~Ferrillo$^{49}$,
M.~Ferro-Luzzi$^{47}$,
S.~Filippov$^{40}$,
R.A.~Fini$^{18}$,
M.~Fiorini$^{20,g}$,
M.~Firlej$^{34}$,
K.M.~Fischer$^{62}$,
C.~Fitzpatrick$^{61}$,
T.~Fiutowski$^{34}$,
F.~Fleuret$^{11,b}$,
M.~Fontana$^{47}$,
F.~Fontanelli$^{23,h}$,
R.~Forty$^{47}$,
V.~Franco~Lima$^{59}$,
M.~Franco~Sevilla$^{65}$,
M.~Frank$^{47}$,
E.~Franzoso$^{20}$,
G.~Frau$^{16}$,
C.~Frei$^{47}$,
D.A.~Friday$^{58}$,
J.~Fu$^{25}$,
Q.~Fuehring$^{14}$,
W.~Funk$^{47}$,
E.~Gabriel$^{31}$,
T.~Gaintseva$^{41}$,
A.~Gallas~Torreira$^{45}$,
D.~Galli$^{19,e}$,
S.~Gallorini$^{27}$,
S.~Gambetta$^{57}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{25}$,
Y.~Gao$^{4}$,
M.~Garau$^{26}$,
L.M.~Garcia~Martin$^{55}$,
P.~Garcia~Moreno$^{44}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{49}$,
B.~Garcia~Plana$^{45}$,
F.A.~Garcia~Rosales$^{11}$,
L.~Garrido$^{44}$,
D.~Gascon$^{44}$,
C.~Gaspar$^{47}$,
R.E.~Geertsema$^{31}$,
D.~Gerick$^{16}$,
L.L.~Gerken$^{14}$,
E.~Gersabeck$^{61}$,
M.~Gersabeck$^{61}$,
T.~Gershon$^{55}$,
D.~Gerstel$^{10}$,
Ph.~Ghez$^{8}$,
V.~Gibson$^{54}$,
A.~Giovent{\`u}$^{45}$,
P.~Gironella~Gironell$^{44}$,
L.~Giubega$^{36}$,
C.~Giugliano$^{20,g}$,
K.~Gizdov$^{57}$,
V.V.~Gligorov$^{12}$,
C.~G{\"o}bel$^{69}$,
E.~Golobardes$^{83}$,
D.~Golubkov$^{38}$,
A.~Golutvin$^{60,80}$,
A.~Gomes$^{1,a}$,
S.~Gomez~Fernandez$^{44}$,
M.~Goncerz$^{33}$,
P.~Gorbounov$^{38}$,
I.V.~Gorelov$^{39}$,
C.~Gotti$^{24}$,
E.~Govorkova$^{31}$,
J.P.~Grabowski$^{16}$,
R.~Graciani~Diaz$^{44}$,
T.~Grammatico$^{12}$,
L.A.~Granado~Cardoso$^{47}$,
E.~Graug{\'e}s$^{44}$,
E.~Graverini$^{48}$,
G.~Graziani$^{21}$,
A.~Grecu$^{36}$,
L.M.~Greeven$^{31}$,
P.~Griffith$^{20}$,
L.~Grillo$^{61}$,
L.~Gruber$^{47}$,
B.R.~Gruberg~Cazon$^{62}$,
C.~Gu$^{3}$,
M.~Guarise$^{20}$,
P. A.~G{\"u}nther$^{16}$,
E.~Gushchin$^{40}$,
A.~Guth$^{13}$,
Yu.~Guz$^{43,47}$,
T.~Gys$^{47}$,
T.~Hadavizadeh$^{68}$,
G.~Haefeli$^{48}$,
C.~Haen$^{47}$,
S.C.~Haines$^{54}$,
P.M.~Hamilton$^{65}$,
Q.~Han$^{7}$,
X.~Han$^{16}$,
T.H.~Hancock$^{62}$,
S.~Hansmann-Menzemer$^{16}$,
N.~Harnew$^{62}$,
T.~Harrison$^{59}$,
C.~Hasse$^{47}$,
M.~Hatch$^{47}$,
J.~He$^{5}$,
M.~Hecker$^{60}$,
K.~Heijhoff$^{31}$,
K.~Heinicke$^{14}$,
A.M.~Hennequin$^{47}$,
K.~Hennessy$^{59}$,
L.~Henry$^{25,46}$,
J.~Heuel$^{13}$,
A.~Hicheur$^{2}$,
D.~Hill$^{62}$,
M.~Hilton$^{61}$,
S.E.~Hollitt$^{14}$,
P.H.~Hopchev$^{48}$,
J.~Hu$^{16}$,
J.~Hu$^{71}$,
W.~Hu$^{7}$,
W.~Huang$^{5}$,
W.~Hulsbergen$^{31}$,
R.J.~Hunter$^{55}$,
M.~Hushchyn$^{81}$,
D.~Hutchcroft$^{59}$,
D.~Hynds$^{31}$,
P.~Ibis$^{14}$,
M.~Idzik$^{34}$,
D.~Ilin$^{37}$,
P.~Ilten$^{52}$,
A.~Inglessi$^{37}$,
K.~Ivshin$^{37}$,
R.~Jacobsson$^{47}$,
S.~Jakobsen$^{47}$,
E.~Jans$^{31}$,
B.K.~Jashal$^{46}$,
A.~Jawahery$^{65}$,
V.~Jevtic$^{14}$,
F.~Jiang$^{3}$,
M.~John$^{62}$,
D.~Johnson$^{47}$,
C.R.~Jones$^{54}$,
T.P.~Jones$^{55}$,
B.~Jost$^{47}$,
N.~Jurik$^{47}$,
S.~Kandybei$^{50}$,
Y.~Kang$^{3}$,
M.~Karacson$^{47}$,
J.M.~Kariuki$^{53}$,
N.~Kazeev$^{81}$,
M.~Kecke$^{16}$,
F.~Keizer$^{54,47}$,
M.~Kenzie$^{55}$,
T.~Ketel$^{32}$,
B.~Khanji$^{47}$,
A.~Kharisova$^{82}$,
S.~Kholodenko$^{43}$,
K.E.~Kim$^{67}$,
T.~Kirn$^{13}$,
V.S.~Kirsebom$^{48}$,
O.~Kitouni$^{63}$,
S.~Klaver$^{31}$,
K.~Klimaszewski$^{35}$,
S.~Koliiev$^{51}$,
A.~Kondybayeva$^{80}$,
A.~Konoplyannikov$^{38}$,
P.~Kopciewicz$^{34}$,
R.~Kopecna$^{16}$,
P.~Koppenburg$^{31}$,
M.~Korolev$^{39}$,
I.~Kostiuk$^{31,51}$,
O.~Kot$^{51}$,
S.~Kotriakhova$^{37}$,
P.~Kravchenko$^{37}$,
L.~Kravchuk$^{40}$,
R.D.~Krawczyk$^{47}$,
M.~Kreps$^{55}$,
F.~Kress$^{60}$,
S.~Kretzschmar$^{13}$,
P.~Krokovny$^{42}$,
W.~Krupa$^{34}$,
W.~Krzemien$^{35}$,
W.~Kucewicz$^{85,33,k}$,
M.~Kucharczyk$^{33}$,
V.~Kudryavtsev$^{42}$,
H.S.~Kuindersma$^{31}$,
G.J.~Kunde$^{66}$,
T.~Kvaratskheliya$^{38}$,
D.~Lacarrere$^{47}$,
G.~Lafferty$^{61}$,
A.~Lai$^{26}$,
A.~Lampis$^{26}$,
D.~Lancierini$^{49}$,
J.J.~Lane$^{61}$,
R.~Lane$^{53}$,
G.~Lanfranchi$^{22}$,
C.~Langenbruch$^{13}$,
J.~Langer$^{14}$,
O.~Lantwin$^{49,80}$,
T.~Latham$^{55}$,
F.~Lazzari$^{28,s}$,
R.~Le~Gac$^{10}$,
S.H.~Lee$^{84}$,
R.~Lef{\`e}vre$^{9}$,
A.~Leflat$^{39}$,
S.~Legotin$^{80}$,
O.~Leroy$^{10}$,
T.~Lesiak$^{33}$,
B.~Leverington$^{16}$,
H.~Li$^{71}$,
L.~Li$^{62}$,
P.~Li$^{16}$,
X.~Li$^{66}$,
Y.~Li$^{6}$,
Y.~Li$^{6}$,
Z.~Li$^{67}$,
X.~Liang$^{67}$,
T.~Lin$^{60}$,
R.~Lindner$^{47}$,
V.~Lisovskyi$^{14}$,
R.~Litvinov$^{26}$,
G.~Liu$^{71}$,
H.~Liu$^{5}$,
S.~Liu$^{6}$,
X.~Liu$^{3}$,
A.~Loi$^{26}$,
J.~Lomba~Castro$^{45}$,
I.~Longstaff$^{58}$,
J.H.~Lopes$^{2}$,
G.~Loustau$^{49}$,
G.H.~Lovell$^{54}$,
Y.~Lu$^{6}$,
D.~Lucchesi$^{27,l}$,
S.~Luchuk$^{40}$,
M.~Lucio~Martinez$^{31}$,
V.~Lukashenko$^{31}$,
Y.~Luo$^{3}$,
A.~Lupato$^{61}$,
E.~Luppi$^{20,g}$,
O.~Lupton$^{55}$,
A.~Lusiani$^{28,q}$,
X.~Lyu$^{5}$,
L.~Ma$^{6}$,
S.~Maccolini$^{19,e}$,
F.~Machefert$^{11}$,
F.~Maciuc$^{36}$,
V.~Macko$^{48}$,
P.~Mackowiak$^{14}$,
S.~Maddrell-Mander$^{53}$,
L.R.~Madhan~Mohan$^{53}$,
O.~Maev$^{37}$,
A.~Maevskiy$^{81}$,
D.~Maisuzenko$^{37}$,
M.W.~Majewski$^{34}$,
S.~Malde$^{62}$,
B.~Malecki$^{47}$,
A.~Malinin$^{79}$,
T.~Maltsev$^{42}$,
H.~Malygina$^{16}$,
G.~Manca$^{26,f}$,
G.~Mancinelli$^{10}$,
R.~Manera~Escalero$^{44}$,
D.~Manuzzi$^{19,e}$,
D.~Marangotto$^{25,n}$,
J.~Maratas$^{9,t}$,
J.F.~Marchand$^{8}$,
U.~Marconi$^{19}$,
S.~Mariani$^{21,21,47}$,
C.~Marin~Benito$^{11}$,
M.~Marinangeli$^{48}$,
P.~Marino$^{48}$,
J.~Marks$^{16}$,
P.J.~Marshall$^{59}$,
G.~Martellotti$^{30}$,
L.~Martinazzoli$^{47}$,
M.~Martinelli$^{24,i}$,
D.~Martinez~Santos$^{45}$,
F.~Martinez~Vidal$^{46}$,
A.~Massafferri$^{1}$,
M.~Materok$^{13}$,
R.~Matev$^{47}$,
A.~Mathad$^{49}$,
Z.~Mathe$^{47}$,
V.~Matiunin$^{38}$,
C.~Matteuzzi$^{24}$,
K.R.~Mattioli$^{84}$,
A.~Mauri$^{31}$,
E.~Maurice$^{11,b}$,
J.~Mauricio$^{44}$,
M.~Mazurek$^{35}$,
M.~McCann$^{60}$,
L.~Mcconnell$^{17}$,
T.H.~Mcgrath$^{61}$,
A.~McNab$^{61}$,
R.~McNulty$^{17}$,
J.V.~Mead$^{59}$,
B.~Meadows$^{64}$,
C.~Meaux$^{10}$,
G.~Meier$^{14}$,
N.~Meinert$^{75}$,
D.~Melnychuk$^{35}$,
S.~Meloni$^{24,i}$,
M.~Merk$^{31,78}$,
A.~Merli$^{25}$,
L.~Meyer~Garcia$^{2}$,
M.~Mikhasenko$^{47}$,
D.A.~Milanes$^{73}$,
E.~Millard$^{55}$,
M.-N.~Minard$^{8}$,
L.~Minzoni$^{20,g}$,
S.E.~Mitchell$^{57}$,
B.~Mitreska$^{61}$,
D.S.~Mitzel$^{47}$,
A.~M{\"o}dden$^{14}$,
R.A.~Mohammed$^{62}$,
R.D.~Moise$^{60}$,
T.~Momb{\"a}cher$^{14}$,
I.A.~Monroy$^{73}$,
S.~Monteil$^{9}$,
M.~Morandin$^{27}$,
G.~Morello$^{22}$,
M.J.~Morello$^{28,q}$,
J.~Moron$^{34}$,
A.B.~Morris$^{74}$,
A.G.~Morris$^{55}$,
R.~Mountain$^{67}$,
H.~Mu$^{3}$,
F.~Muheim$^{57}$,
M.~Mukherjee$^{7}$,
M.~Mulder$^{47}$,
D.~M{\"u}ller$^{47}$,
K.~M{\"u}ller$^{49}$,
C.H.~Murphy$^{62}$,
D.~Murray$^{61}$,
P.~Muzzetto$^{26}$,
P.~Naik$^{53}$,
T.~Nakada$^{48}$,
R.~Nandakumar$^{56}$,
T.~Nanut$^{48}$,
I.~Nasteva$^{2}$,
M.~Needham$^{57}$,
I.~Neri$^{20,g}$,
N.~Neri$^{25,n}$,
S.~Neubert$^{74}$,
N.~Neufeld$^{47}$,
R.~Newcombe$^{60}$,
T.D.~Nguyen$^{48}$,
C.~Nguyen-Mau$^{48}$,
E.M.~Niel$^{11}$,
S.~Nieswand$^{13}$,
N.~Nikitin$^{39}$,
N.S.~Nolte$^{47}$,
C.~Nunez$^{84}$,
A.~Oblakowska-Mucha$^{34}$,
V.~Obraztsov$^{43}$,
D.P.~O'Hanlon$^{53}$,
R.~Oldeman$^{26,f}$,
C.J.G.~Onderwater$^{77}$,
A.~Ossowska$^{33}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{38}$,
P.~Owen$^{49}$,
A.~Oyanguren$^{46}$,
B.~Pagare$^{55}$,
P.R.~Pais$^{47}$,
T.~Pajero$^{28,47,q}$,
A.~Palano$^{18}$,
M.~Palutan$^{22}$,
Y.~Pan$^{61}$,
G.~Panshin$^{82}$,
A.~Papanestis$^{56}$,
M.~Pappagallo$^{57}$,
L.L.~Pappalardo$^{20,g}$,
C.~Pappenheimer$^{64}$,
W.~Parker$^{65}$,
C.~Parkes$^{61}$,
C.J.~Parkinson$^{45}$,
B.~Passalacqua$^{20}$,
G.~Passaleva$^{21}$,
A.~Pastore$^{18}$,
M.~Patel$^{60}$,
C.~Patrignani$^{19,e}$,
C.J.~Pawley$^{78}$,
A.~Pearce$^{47}$,
A.~Pellegrino$^{31}$,
M.~Pepe~Altarelli$^{47}$,
S.~Perazzini$^{19}$,
D.~Pereima$^{38}$,
P.~Perret$^{9}$,
K.~Petridis$^{53}$,
A.~Petrolini$^{23,h}$,
A.~Petrov$^{79}$,
S.~Petrucci$^{57}$,
M.~Petruzzo$^{25}$,
A.~Philippov$^{41}$,
L.~Pica$^{28}$,
M.~Piccini$^{76}$,
B.~Pietrzyk$^{8}$,
G.~Pietrzyk$^{48}$,
M.~Pili$^{62}$,
D.~Pinci$^{30}$,
J.~Pinzino$^{47}$,
F.~Pisani$^{47}$,
A.~Piucci$^{16}$,
Resmi ~P.K$^{10}$,
V.~Placinta$^{36}$,
S.~Playfer$^{57}$,
J.~Plews$^{52}$,
M.~Plo~Casasus$^{45}$,
F.~Polci$^{12}$,
M.~Poli~Lener$^{22}$,
M.~Poliakova$^{67}$,
A.~Poluektov$^{10}$,
N.~Polukhina$^{80,c}$,
I.~Polyakov$^{67}$,
E.~Polycarpo$^{2}$,
G.J.~Pomery$^{53}$,
S.~Ponce$^{47}$,
A.~Popov$^{43}$,
D.~Popov$^{5,47}$,
S.~Popov$^{41}$,
S.~Poslavskii$^{43}$,
K.~Prasanth$^{33}$,
L.~Promberger$^{47}$,
C.~Prouve$^{45}$,
V.~Pugatch$^{51}$,
A.~Puig~Navarro$^{49}$,
H.~Pullen$^{62}$,
G.~Punzi$^{28,m}$,
W.~Qian$^{5}$,
J.~Qin$^{5}$,
R.~Quagliani$^{12}$,
B.~Quintana$^{8}$,
N.V.~Raab$^{17}$,
R.I.~Rabadan~Trejo$^{10}$,
B.~Rachwal$^{34}$,
J.H.~Rademacker$^{53}$,
M.~Rama$^{28}$,
M.~Ramos~Pernas$^{55}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{41,81}$,
G.~Raven$^{32}$,
M.~Reboud$^{8}$,
F.~Redi$^{48}$,
F.~Reiss$^{12}$,
C.~Remon~Alepuz$^{46}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{62}$,
R.~Ribatti$^{28}$,
S.~Ricciardi$^{56}$,
D.S.~Richards$^{56}$,
K.~Rinnert$^{59}$,
P.~Robbe$^{11}$,
A.~Robert$^{12}$,
G.~Robertson$^{57}$,
A.B.~Rodrigues$^{48}$,
E.~Rodrigues$^{59}$,
J.A.~Rodriguez~Lopez$^{73}$,
A.~Rollings$^{62}$,
P.~Roloff$^{47}$,
V.~Romanovskiy$^{43}$,
M.~Romero~Lamas$^{45}$,
A.~Romero~Vidal$^{45}$,
J.D.~Roth$^{84}$,
M.~Rotondo$^{22}$,
M.S.~Rudolph$^{67}$,
T.~Ruf$^{47}$,
J.~Ruiz~Vidal$^{46}$,
A.~Ryzhikov$^{81}$,
J.~Ryzka$^{34}$,
J.J.~Saborido~Silva$^{45}$,
N.~Sagidova$^{37}$,
N.~Sahoo$^{55}$,
B.~Saitta$^{26,f}$,
C.~Sanchez~Gras$^{31}$,
C.~Sanchez~Mayordomo$^{46}$,
R.~Santacesaria$^{30}$,
C.~Santamarina~Rios$^{45}$,
M.~Santimaria$^{22}$,
E.~Santovetti$^{29,j}$,
D.~Saranin$^{80}$,
G.~Sarpis$^{61}$,
M.~Sarpis$^{74}$,
A.~Sarti$^{30}$,
C.~Satriano$^{30,p}$,
A.~Satta$^{29}$,
M.~Saur$^{5}$,
D.~Savrina$^{38,39}$,
H.~Sazak$^{9}$,
L.G.~Scantlebury~Smead$^{62}$,
S.~Schael$^{13}$,
M.~Schellenberg$^{14}$,
M.~Schiller$^{58}$,
H.~Schindler$^{47}$,
M.~Schmelling$^{15}$,
T.~Schmelzer$^{14}$,
B.~Schmidt$^{47}$,
O.~Schneider$^{48}$,
A.~Schopper$^{47}$,
M.~Schubiger$^{31}$,
S.~Schulte$^{48}$,
M.H.~Schune$^{11}$,
R.~Schwemmer$^{47}$,
B.~Sciascia$^{22}$,
A.~Sciubba$^{30}$,
S.~Sellam$^{45}$,
A.~Semennikov$^{38}$,
A.~Sergi$^{52,47}$,
N.~Serra$^{49}$,
J.~Serrano$^{10}$,
L.~Sestini$^{27}$,
A.~Seuthe$^{14}$,
P.~Seyfert$^{47}$,
D.M.~Shangase$^{84}$,
M.~Shapkin$^{43}$,
I.~Shchemerov$^{80}$,
L.~Shchutska$^{48}$,
T.~Shears$^{59}$,
L.~Shekhtman$^{42}$,
V.~Shevchenko$^{79}$,
E.B.~Shields$^{24,i}$,
E.~Shmanin$^{80}$,
J.D.~Shupperd$^{67}$,
B.G.~Siddi$^{20}$,
R.~Silva~Coutinho$^{49}$,
G.~Simi$^{27}$,
S.~Simone$^{18,d}$,
I.~Skiba$^{20,g}$,
N.~Skidmore$^{74}$,
T.~Skwarnicki$^{67}$,
M.W.~Slater$^{52}$,
J.C.~Smallwood$^{62}$,
J.G.~Smeaton$^{54}$,
A.~Smetkina$^{38}$,
E.~Smith$^{13}$,
M.~Smith$^{60}$,
A.~Snoch$^{31}$,
M.~Soares$^{19}$,
L.~Soares~Lavra$^{9}$,
M.D.~Sokoloff$^{64}$,
F.J.P.~Soler$^{58}$,
A.~Solovev$^{37}$,
I.~Solovyev$^{37}$,
F.L.~Souza~De~Almeida$^{2}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{14}$,
E.~Spadaro~Norella$^{25,n}$,
P.~Spradlin$^{58}$,
F.~Stagni$^{47}$,
M.~Stahl$^{64}$,
S.~Stahl$^{47}$,
P.~Stefko$^{48}$,
O.~Steinkamp$^{49,80}$,
S.~Stemmle$^{16}$,
O.~Stenyakin$^{43}$,
H.~Stevens$^{14}$,
S.~Stone$^{67}$,
S.~Stracka$^{28}$,
M.E.~Stramaglia$^{48}$,
M.~Straticiuc$^{36}$,
D.~Strekalina$^{80}$,
S.~Strokov$^{82}$,
F.~Suljik$^{62}$,
J.~Sun$^{26}$,
L.~Sun$^{72}$,
Y.~Sun$^{65}$,
P.~Svihra$^{61}$,
P.N.~Swallow$^{52}$,
K.~Swientek$^{34}$,
A.~Szabelski$^{35}$,
T.~Szumlak$^{34}$,
M.~Szymanski$^{47}$,
S.~Taneja$^{61}$,
Z.~Tang$^{3}$,
T.~Tekampe$^{14}$,
F.~Teubert$^{47}$,
E.~Thomas$^{47}$,
K.A.~Thomson$^{59}$,
M.J.~Tilley$^{60}$,
V.~Tisserand$^{9}$,
S.~T'Jampens$^{8}$,
M.~Tobin$^{6}$,
S.~Tolk$^{47}$,
L.~Tomassetti$^{20,g}$,
D.~Torres~Machado$^{1}$,
D.Y.~Tou$^{12}$,
M.~Traill$^{58}$,
M.T.~Tran$^{48}$,
E.~Trifonova$^{80}$,
C.~Trippl$^{48}$,
A.~Tsaregorodtsev$^{10}$,
G.~Tuci$^{28,m}$,
A.~Tully$^{48}$,
N.~Tuning$^{31}$,
A.~Ukleja$^{35}$,
D.J.~Unverzagt$^{16}$,
A.~Usachov$^{31}$,
A.~Ustyuzhanin$^{41,81}$,
U.~Uwer$^{16}$,
A.~Vagner$^{82}$,
V.~Vagnoni$^{19}$,
A.~Valassi$^{47}$,
G.~Valenti$^{19}$,
M.~van~Beuzekom$^{31}$,
H.~Van~Hecke$^{66}$,
E.~van~Herwijnen$^{80}$,
C.B.~Van~Hulse$^{17}$,
M.~van~Veghel$^{77}$,
R.~Vazquez~Gomez$^{45}$,
P.~Vazquez~Regueiro$^{45}$,
C.~V{\'a}zquez~Sierra$^{31}$,
S.~Vecchi$^{20}$,
J.J.~Velthuis$^{53}$,
M.~Veltri$^{21,o}$,
A.~Venkateswaran$^{67}$,
M.~Veronesi$^{31}$,
M.~Vesterinen$^{55}$,
D.~Vieira$^{64}$,
M.~Vieites~Diaz$^{48}$,
H.~Viemann$^{75}$,
X.~Vilasis-Cardona$^{83}$,
E.~Vilella~Figueras$^{59}$,
P.~Vincent$^{12}$,
G.~Vitali$^{28}$,
A.~Vollhardt$^{49}$,
D.~Vom~Bruch$^{12}$,
A.~Vorobyev$^{37}$,
V.~Vorobyev$^{42}$,
N.~Voropaev$^{37}$,
R.~Waldi$^{75}$,
J.~Walsh$^{28}$,
C.~Wang$^{16}$,
J.~Wang$^{3}$,
J.~Wang$^{72}$,
J.~Wang$^{4}$,
J.~Wang$^{6}$,
M.~Wang$^{3}$,
R.~Wang$^{53}$,
Y.~Wang$^{7}$,
Z.~Wang$^{49}$,
D.R.~Ward$^{54}$,
H.M.~Wark$^{59}$,
N.K.~Watson$^{52}$,
S.G.~Weber$^{12}$,
D.~Websdale$^{60}$,
C.~Weisser$^{63}$,
B.D.C.~Westhenry$^{53}$,
D.J.~White$^{61}$,
M.~Whitehead$^{53}$,
D.~Wiedner$^{14}$,
G.~Wilkinson$^{62}$,
M.~Wilkinson$^{67}$,
I.~Williams$^{54}$,
M.~Williams$^{63,68}$,
M.R.J.~Williams$^{57}$,
F.F.~Wilson$^{56}$,
W.~Wislicki$^{35}$,
M.~Witek$^{33}$,
L.~Witola$^{16}$,
G.~Wormser$^{11}$,
S.A.~Wotton$^{54}$,
H.~Wu$^{67}$,
K.~Wyllie$^{47}$,
Z.~Xiang$^{5}$,
D.~Xiao$^{7}$,
Y.~Xie$^{7}$,
H.~Xing$^{71}$,
A.~Xu$^{4}$,
J.~Xu$^{5}$,
L.~Xu$^{3}$,
M.~Xu$^{7}$,
Q.~Xu$^{5}$,
Z.~Xu$^{4}$,
D.~Yang$^{3}$,
Y.~Yang$^{5}$,
Z.~Yang$^{3}$,
Z.~Yang$^{65}$,
Y.~Yao$^{67}$,
L.E.~Yeomans$^{59}$,
H.~Yin$^{7}$,
J.~Yu$^{70}$,
X.~Yuan$^{67}$,
O.~Yushchenko$^{43}$,
K.A.~Zarebski$^{52}$,
M.~Zavertyaev$^{15,c}$,
M.~Zdybal$^{33}$,
O.~Zenaiev$^{47}$,
M.~Zeng$^{3}$,
D.~Zhang$^{7}$,
L.~Zhang$^{3}$,
S.~Zhang$^{4}$,
Y.~Zhang$^{47}$,
A.~Zhelezov$^{16}$,
Y.~Zheng$^{5}$,
X.~Zhou$^{5}$,
Y.~Zhou$^{5}$,
X.~Zhu$^{3}$,
V.~Zhukov$^{13,39}$,
J.B.~Zonneveld$^{57}$,
S.~Zucchelli$^{19,e}$,
D.~Zuliani$^{27}$,
G.~Zunica$^{61}$.\bigskip

{\footnotesize \it

$ ^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$ ^{5}$University of Chinese Academy of Sciences, Beijing, China\\
$ ^{6}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$ ^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$ ^{8}$Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$ ^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$ ^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$ ^{12}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$ ^{13}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$ ^{14}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$ ^{15}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{16}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$ ^{17}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{18}$INFN Sezione di Bari, Bari, Italy\\
$ ^{19}$INFN Sezione di Bologna, Bologna, Italy\\
$ ^{20}$INFN Sezione di Ferrara, Ferrara, Italy\\
$ ^{21}$INFN Sezione di Firenze, Firenze, Italy\\
$ ^{22}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$ ^{23}$INFN Sezione di Genova, Genova, Italy\\
$ ^{24}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$ ^{25}$INFN Sezione di Milano, Milano, Italy\\
$ ^{26}$INFN Sezione di Cagliari, Monserrato, Italy\\
$ ^{27}$Universita degli Studi di Padova, Universita e INFN, Padova, Padova, Italy\\
$ ^{28}$INFN Sezione di Pisa, Pisa, Italy\\
$ ^{29}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$ ^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$ ^{31}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$ ^{32}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$ ^{33}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$ ^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$ ^{35}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{36}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{37}$Petersburg Nuclear Physics Institute NRC Kurchatov Institute (PNPI NRC KI), Gatchina, Russia\\
$ ^{38}$Institute of Theoretical and Experimental Physics NRC Kurchatov Institute (ITEP NRC KI), Moscow, Russia, Moscow, Russia\\
$ ^{39}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{40}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$ ^{41}$Yandex School of Data Analysis, Moscow, Russia\\
$ ^{42}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$ ^{43}$Institute for High Energy Physics NRC Kurchatov Institute (IHEP NRC KI), Protvino, Russia, Protvino, Russia\\
$ ^{44}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$ ^{45}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{46}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$ ^{47}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{48}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{49}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$ ^{50}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{51}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{52}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{53}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{54}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{55}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{56}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{57}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{58}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{59}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{60}$Imperial College London, London, United Kingdom\\
$ ^{61}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{62}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{63}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{64}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{65}$University of Maryland, College Park, MD, United States\\
$ ^{66}$Los Alamos National Laboratory (LANL), Los Alamos, United States\\
$ ^{67}$Syracuse University, Syracuse, NY, United States\\
$ ^{68}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{55}$\\
$ ^{69}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{70}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$ ^{71}$Guangdong Provencial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$ ^{72}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$ ^{73}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{12}$\\
$ ^{74}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{16}$\\
$ ^{75}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{16}$\\
$ ^{76}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{20}$\\
$ ^{77}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{31}$\\
$ ^{78}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{31}$\\
$ ^{79}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{38}$\\
$ ^{80}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{38}$\\
$ ^{81}$National Research University Higher School of Economics, Moscow, Russia, associated to $^{41}$\\
$ ^{82}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{38}$\\
$ ^{83}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{44}$\\
$ ^{84}$University of Michigan, Ann Arbor, United States, associated to $^{67}$\\
$ ^{85}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Laboratoire Leprince-Ringuet, Palaiseau, France\\
$^{c}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$^{d}$Universit{\`a} di Bari, Bari, Italy\\
$^{e}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{f}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{g}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{h}$Universit{\`a} di Genova, Genova, Italy\\
$^{i}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{j}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{k}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
$^{l}$Universit{\`a} di Padova, Padova, Italy\\
$^{m}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{n}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{o}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{p}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{q}$Scuola Normale Superiore, Pisa, Italy\\
$^{r}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{s}$Universit{\`a} di Siena, Siena, Italy\\
$^{t}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$^{u}$Novosibirsk State University, Novosibirsk, Russia\\
$^{v}$INFN Sezione di Trieste, Trieste, Italy\\
\medskip
}
\end{flushleft}

==> LHCb_Authorship_DD-MMM-20YY.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> acknowledgements_intro.tex <==
\section{Acknowledgements paragraph}

Include the following text in the Acknowledgements section in all paper
drafts. It is not needed for analysis notes or conference reports.

The text below are the acknowledgements as approved by the collaboration
board. Extending the acknowledgements to include individuals from outside the
collaboration who have contributed to the analysis should be approved by the
EB. The extra acknowledgements are normally placed before the standard 
acknowledgements, unless it matches better with the text of the standard 
acknowledgements to put them elsewhere. They should be included in the draft 
for the first circulation. Except in exceptional circumstances, to be approved by the
EB chair, authors of the paper should not be named in extended acknowledgements.

%\vspace{1cm}

\input{acknowledgements}


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub \\
\texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum \\
\texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb \\
\texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chic} & \chic & \texttt{\textbackslash chiczero} & \chiczero \\
\texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash chicJ} & \chicJ \\
\texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero & \texttt{\textbackslash chibone} & \chibone \\
\texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresz} & \Xiresz \\
\texttt{\textbackslash Xiresm} & \Xiresm & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xiresbarz} & \Xiresbarz \\
\texttt{\textbackslash Xiresbarp} & \Xiresbarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xic} & \Xic \\
\texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar \\
\texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac \\
\texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar \\
\texttt{\textbackslash Xiccp} & \Xiccp & \texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm \\
\texttt{\textbackslash Xiccbarmm} & \Xiccbarmm & \texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar \\
\texttt{\textbackslash Omegaccc} & \Omegaccc & \texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units (these macros add a small space in front)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}   } & \unit{kg}    &  \\
\end{tabular*}

\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash mevc} & \mevc \\
\texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc & \texttt{\textbackslash gevcc} & \gevcc \\
\texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc &  \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa

